CIAR: Interval-based Collaborative Decoding for Image Generation Acceleration

Auto-regressive (AR) models have recently made notable progress in image generation, achieving performance comparable to diffusion-based approaches. However, their computational intensity and sequential nature impede on-device deployment, causing disruptive latency. We address this via a cloud-device collaboration framework \textbf{CIAR}, which utilizes on-device self-verification to handle two key properties of visual synthesis: \textit{the vast token vocabulary} required for high-fidelity images and \textit{inherent spatial redundancy} which leads to extreme predictability in homogeneous regions, while object boundaries exhibit high uncertainty. Uniform verification wastes resources on such redundant tokens. Our solution centers on an on-device token uncertainty quantifier, which adopts continuous probability intervals to accelerate processing and make it feasible for large visual vocabularies instead of conventional discrete solution sets. Additionally, we incorporate a Interval-enhanced decoding module to further speed up decoding while maintaining visual fidelity and semantic consistency via a distribution alignment training strategy. Extensive experiments demonstrate that CIAR achieves a 2.18x speed-up and reduces cloud requests by 70\%, while preserving image quality compared to existing methods.

==> tables/discrete_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[t]
% \centering
% \caption{Ablation: Discrete vs Continuous}
% \begin{tabular}{c|c|ccc}
% \toprule[2pt]
%                                    &                                     & \multicolumn{3}{c}{\textbf{Metric}}                                                                                                         \\ \cmidrule{3-5} 
% \multirow{-2}{*}{\textbf{Methods}} & \multirow{-2}{*}{\textbf{Settings}} & \multicolumn{1}{c|}{\textbf{CLIP (↑)}}              & \multicolumn{1}{c|}{\textbf{FID (↓)}}                & \textbf{Latency(s / image)}    \\ \midrule \midrule
%                                    & k = 100                             & \multicolumn{1}{c|}{0.3081}                         & \multicolumn{1}{c|}{26.0371}                         & 15.3195                        \\
%                                    & k = 200                             & \multicolumn{1}{c|}{0.3096}                         & \multicolumn{1}{c|}{25.5508}                         & 95.7704                        \\
%                                    & k = 300                             & \multicolumn{1}{c|}{0.3123}                         & \multicolumn{1}{c|}{24.8237}                         & 400.4220                       \\
% \multirow{-4}{*}{Discrete}         & k = 400                             & \multicolumn{1}{c|}{placeholder}                    & \multicolumn{1}{c|}{placeholder}                     & 1001.5600                      \\ \hline
% Continuous                         & \cellcolor[HTML]{F2F2FF}Ours        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2FF}0.3176} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2FF}24.2463} & \cellcolor[HTML]{F2F2FF}4.7240 \\
% \bottomrule[2pt]
% \end{tabular}
% \end{table}

\begin{table}[t]
\centering
\caption{Ablation: Discrete vs Continuous}
\begin{tabular}{c|c|cc}
\toprule[2pt]
                                   &                                     & \multicolumn{2}{c}{\textbf{Metric}}                                                                        \\ \cmidrule{3-5} 
\multirow{-2}{*}{\textbf{Methods}} & \multirow{-2}{*}{\textbf{Settings}} & \multicolumn{1}{c|}{\textbf{CLIP (↑)}}              & \multicolumn{1}{c|}{\textbf{FID (↓)}}                \\ \midrule \midrule
                                   & k = 100                             & \multicolumn{1}{c|}{0.3081}                         & \multicolumn{1}{c|}{26.0371}                         \\
                                   & k = 200                             & \multicolumn{1}{c|}{0.3096}                         & \multicolumn{1}{c|}{25.5508}                         \\
                                   & k = 300                             & \multicolumn{1}{c|}{0.3123}                         & \multicolumn{1}{c|}{24.8237}                         \\
\multirow{-4}{*}{Discrete}         & k = 400                             & \multicolumn{1}{c|}{placeholder}                    & \multicolumn{1}{c|}{placeholder}                     \\ \hline
Continuous                         & \cellcolor[HTML]{F2F2FF}Ours        & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2FF}0.3176} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2FF}24.2463} \\ \hline
\bottomrule[2pt]
\end{tabular}
\end{table}
